Concurrent CPU-GPU Task Programming using Modern C++

In this paper, we introduce Heteroflow, a new C++ library to help developers quickly write parallel CPU-GPU programs using task dependency graphs. Heteroflow leverages the power of modern C++ and task-based approaches to enable efficient implementations of heterogeneous decomposition strategies. Our new CPU-GPU programming model allows users to express a problem in a way that adapts to effective separation of concerns and expertise encapsulation. Compared with existing libraries, Heteroflow is more cost-efficient in performance scaling, programming productivity, and solution generality. We have evaluated Heteroflow on two real applications in VLSI design automation and demonstrated the performance scalability across different CPU-GPU numbers and problem sizes. At a particular example of VLSI timing analysis with million-scale tasking, Heteroflow achieved 7.7x runtime speed-up (99 vs 13 minutes) over a baseline on a machine of 40 CPU cores and 4 GPUs.

==> Fig/exp-placement/exp-placement-2.tex <==
\begin{figure}[h]
  \centering

  \pgfplotsset{
    title style={font=\Large},
    label style={font=\Large},
    %ylabel style={rotate=-90},
  }
  %
  \begin{tikzpicture}[scale=0.50]
    \begin{axis}[
      title=Runtime vs Problem Size (40 cores),
      xlabel=Problem Size (\# iterations),
      ylabel=Runtime (seconds),
      legend pos=north west,
    ]
    \addplot+ table[x=N,y=four-gpus,col sep=space]{Fig/exp-placement/weak-scalability-gpu.csv};
    \addplot+ table[x=N,y=three-gpus,col sep=space]{Fig/exp-placement/weak-scalability-gpu.csv};
    \addplot+ table[x=N,y=two-gpus,col sep=space]{Fig/exp-placement/weak-scalability-gpu.csv};
    \addplot+ table[x=N,y=one-gpu,col sep=space]{Fig/exp-placement/weak-scalability-gpu.csv};
    \legend{4 GPUs, 3 GPUs, 2 GPUs, 1 GPU}
    \end{axis}
  \end{tikzpicture}
  %
  \begin{tikzpicture}[scale=0.50]
    \begin{axis}[
      title=Runtime vs Problem Size (4 GPUs),
      xlabel=Problem Size (\# iterations),
      ylabel=Runtime (seconds),
      legend pos=north west,
    ]
    \addplot+ table[x=N,y=40,col sep=space]{Fig/exp-placement/weak-scalability-cpu.csv};
    \addplot+ table[x=N,y=32,col sep=space]{Fig/exp-placement/weak-scalability-cpu.csv};
    \addplot+ table[x=N,y=24,col sep=space]{Fig/exp-placement/weak-scalability-cpu.csv};
    \addplot+ table[x=N,y=16,col sep=space]{Fig/exp-placement/weak-scalability-cpu.csv};
    \addplot+ table[x=N,y=8,col sep=space]{Fig/exp-placement/weak-scalability-cpu.csv};
    \legend{40 Cores, 32 Cores, 24 Cores, 16 Cores, 8 Cores}
    \end{axis}
  \end{tikzpicture}
  %
  \caption{Runtimes at different CPU-GPU numbers and problem sizes on placing the circuit bigblue4 (2.2M cells and 2.2M nets).}
  \label{fig::exp-placement-weak-scaling}
\end{figure}



==> Fig/exp-timing/exp-timing-2.tex <==
\begin{figure}[h]
  \centering

  \pgfplotsset{
    title style={font=\Large},
    label style={font=\Large},
    %ylabel style={rotate=-90},
  }
  %
  \begin{tikzpicture}[scale=0.50]
    \begin{axis}[
      title=Runtime vs Problem Size (40 cores),
      xlabel=Problem Size (\# analysis views),
      ylabel=Runtime (minutes),
      legend pos=north west,
    ]
    \addplot+ table[x=N,y=four-gpus,col sep=space]{Fig/exp-timing/weak-scalability-gpu.csv};
    \addplot+ table[x=N,y=three-gpus,col sep=space]{Fig/exp-timing/weak-scalability-gpu.csv};
    \addplot+ table[x=N,y=two-gpus,col sep=space]{Fig/exp-timing/weak-scalability-gpu.csv};
    \addplot+ table[x=N,y=one-gpu,col sep=space]{Fig/exp-timing/weak-scalability-gpu.csv};
    \legend{4 GPUs, 3 GPUs, 2 GPUs, 1 GPU}
    \end{axis}
  \end{tikzpicture}
  %
  \begin{tikzpicture}[scale=0.50]
    \begin{axis}[
      title=Runtime vs Problem Size (4 GPUs),
      xlabel=Problem Size (\# analysis views),
      ylabel=Runtime (minutes),
      legend pos=north west,
    ]
    \addplot+ table[x=N,y=40,col sep=space]{Fig/exp-timing/weak-scalability-cpu.csv};
    \addplot+ table[x=N,y=32,col sep=space]{Fig/exp-timing/weak-scalability-cpu.csv};
    \addplot+ table[x=N,y=24,col sep=space]{Fig/exp-timing/weak-scalability-cpu.csv};
    \addplot+ table[x=N,y=16,col sep=space]{Fig/exp-timing/weak-scalability-cpu.csv};
    \addplot+ table[x=N,y=8,col sep=space]{Fig/exp-timing/weak-scalability-cpu.csv};
    \legend{40 Cores, 32 Cores, 24 Cores, 16 Cores, 8 Cores}
    \end{axis}
  \end{tikzpicture}
  %
  \caption{Runtimes at different CPU-GPU numbers and problem sizes on analyzing the circuit netcard (1.5M gates and 1.5M nets).}
  \label{fig::exp-timing-weak-scaling}
\end{figure}


